RTAMT -- Runtime Robustness Monitors with Application to CPS and Robotics

In this paper, we present Real-Time Analog Monitoring Tool (RTAMT), a tool for quantitative monitoring of Signal Temporal Logic (STL) specifications. The library implements a flexible architecture that supports: (1) various environments connected by an Application Programming Interface (API) in Python, (2) various flavors of temporal logic specification and robustness notion such as STL, including an interface-aware variant that distinguishes between input and output variables, and (3) discrete-time and dense-time interpretation of STL with generation of online and offline monitors. We specifically focus on robotics and Cyber-Physical Systems (CPSs) applications, showing how to integrate RTAMT with (1) the Robot Operating System (ROS) and (2) MATLAB/Simulink environments. We evaluate the tool by demonstrating several use scenarios involving service robotic and avionic applications.

==> figures/lib.tex <==
\begin{picture}(0,0)
    \includegraphics{lib.pdf}
\end{picture}
\setlength{\unitlength}{3947sp}

\begingroup\makeatletter\ifx\SetFigFont\undefined
\gdef\SetFigFont#1#2#3#4#5{
    \reset@font\fontsize{#1}{#2pt}
    \fontfamily{#3}\fontseries{#4}\fontshape{#5}
    \selectfont}
\fi\endgroup

\begin{picture}(8166,6816)(2968,-8494)
    \put(6751,-3586){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$in_m$}
    }}}}
    \put(3451,-3136){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$update(index,[(in_1,val_1),\ldots,(in_m,val_m)])$}
    }}}}
    \put(5701,-3736){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cdots$}
    }}}}
    \put(4651,-3586){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$in_1$}
    }}}}
    \put(3751,-3586){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$out$}
    }}}}
    \put(4651,-3886){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$val_1$}
    }}}}
    \put(3751,-3886){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$val$}
    }}}}
    \put(6751,-3886){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$val_m$}
    }}}}
    \put(3451,-2836){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$parse()$}
    }}}}
    \put(3451,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$get\_spec\_from\_file(filename)$}
    }}}}
\end{picture}


==> figures/ros.tex <==
\begin{picture}(0,0)
    \includegraphics{figures/ros.pdf}
\end{picture}
\setlength{\unitlength}{3947sp}

\begingroup\makeatletter\ifx\SetFigFont\undefined
\gdef\SetFigFont#1#2#3#4#5{
    \reset@font\fontsize{#1}{#2pt}
    \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
    \selectfont}
\fi\endgroup

\begin{picture}(6366,4566)(1768,-6394)
    \put(2626,-4486){\makebox(0,0)[rb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$req$}
    }}}}
    \put(3376,-4036){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$gnt$}
    }}}}
    \put(7351,-5536){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$out$}
    }}}}
    \put(7726,-5086){\rotatebox{90.0}{\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$out = \globally(req \geq 3 \rightarrow \finally_I gnt \geq 3)$}
    }}}}}
\end{picture}

==> figures/stl-translator.tex <==
\begin{picture}(0,0)
    \includegraphics{figures/stl-translator.pdf}
\end{picture}
\setlength{\unitlength}{3947sp}

\begingroup\makeatletter\ifx\SetFigFont\undefined
\gdef\SetFigFont#1#2#3#4#5{
    \reset@font\fontsize{#1}{#2pt}
    \fontfamily{#3}\fontseries{#4}\fontshape{#5}
    \selectfont}
\fi\endgroup

\begin{picture}(8745,2766)(2068,-11794)
\end{picture}

==> reviews/memo3.tex <==
Section 3 is getting much better. There are still some room for improvement:

- In the definition of a discrete and dense-time signal: I do not see a need for defining the sequence of timestamps J, T and values V, I think it is sufficient to define ideal (finite) discrete and dense signals as (partial) functions from N (for discrete signals) and R (for dense signals) to R^n. I think that talking about the sequence of timestamps and values makes sense only when we start talking about the actual representation of signals and interpolation functions.

- I would suggest defining first the most general STL, that is with bounded and unbounded operators, and with future and past, and only then say that in particular, we focus on the bounded future and pure past fragment. The reason is that for the offline monitors, we support the most general version of STL, and the bounded future + past fragments are needed mainly for the online monitors.

    not phi
    phi1 or phi2
    phi1 until_I phi2
    phi1 S_I phi2
    where I is of the form [a,b], [a,\inf)
    bounded STL is the above subset where phi1 U_I phi2 is restricted to
    I=[a,b]
    you cannot have I=[a, inf)
    past STL is STL without U_I
    bounded-future STL = past STL + future STL with only U_[a,b] operator

